Photometric, kinematic and variability study in the young open cluster NGC 1960

We present a comprehensive photometric analysis of a young open cluster NGC 1960 (M36) along with the long-term variability study of this cluster. Based on the kinematic data of Gaia DR2, the membership probabilities of 3871 stars are ascertained in the cluster field among which 262 stars are found to be cluster members. Considering the kinematic and trigonometric measurements of the cluster members, we estimate a mean cluster parallax of 0.86+/-0.05 mas and mean proper motions of mu_RA = -0.143+/-0.008 mas/yr, mu_Dec = -3.395+/-0.008 mas/yr. We obtain basic parameters of the cluster such as E(B-V) = 0.24+/-0.02 mag, log(Age/yr)=7.44+/-0.02, and distance = 1.17+/-0.06 kpc. The mass function slope in the cluster for the stars in the mass range of 0.72-7.32 M_solar is found to be \gamma = -1.26+/-0.19. We find that mass segregation is still taking place in the cluster which is yet to be dynamically relaxed. This work also presents first high-precision variability survey in the central 13'x13' among which 72 are periodic variables. Among them, 59 are short-period (P<1 day)and 13 are long-period (P>1 day). The variable stars have V magnitudes ranging between 9.1 to 19.4 mag and periods between 41 minutes to 10.74 days. On the basis of their locations in the H-R diagram, periods and characteristic light curves, the 20 periodic variables belong to the cluster. We classified them as 2 delta-Scuti, 3 gamma-Dor, 2 slowly pulsating B stars, 5 rotational variables, 2 non-pulsating B stars and 6 as miscellaneous variables.

==> bibliography.tex <==
\begin{thebibliography}{}

\bibitem[Barkhatatova et al.(1985)Barkhatatova et al.]{1985AZ...62..854B}
  Barkhatova K.~A., Zokharova P.~E., Shaskina L.~P. {\&} Oreknova L.~K., 1985, Astron. Zh., 62, 854

\bibitem[Bonnell et al.(2003)Bonnell, Bate \& Vine]{2003MNRAS...343..413B}
  Bonnel I.~A., Bate M.~R. {\&} Vine S.~G., 2003, MNRAS, 343, 413

\bibitem[Cardelli et al.(1989)Cardelli et al.]{1989APJ...345..245C}
Cardelli J.~A., Clayton G.~C. {\&} Mathis J.~S., 1989, ApJ, 345, 245

\bibitem[Chian \& Zhu(1966)Chian \& Zhu]{1966AS...26..53C}
  Chian B. {\&} Zhu G., 1966, Ann. Shesan G. Sect. of Shanghai Obs., 26, 53
  
\bibitem[Chini \& Wargue(1990)Chini \& Wargue]{1990AA...227..5C}
  Chini R. {\&} Wargue W.~F., 1990, A{\&}A, 227, 5

\bibitem[Hasan et al.(2005)Hasan et al.]{2005BASI...33..151H}
  Hasan P., Kilambi G.~C. \& Hasan S.~N., 2005, Bull. Astr. Soc. India, 33, 151
  
\bibitem[Hoyle et al.(2003)Hoyle et al.]{2003MNRAS...345..269H}
 Hoyle F., Shankes T. {\&} Tanvir N.~R., 2003, MNRAS, 345, 269

\bibitem[Jeffries et al.(2013)Jeffries et al.]{2013MNRAS...434..2438J}
  Jeffries R.~D., Naylor R., Mayne N.~J., Bell C.~P.~M. {\&} Littlefair S.~P., 2013, MNRAS, 434, 2438

\bibitem[Johnson \& Morgan (1953)Johnson \& Morgan]{1953AP...117..313J}
  Johnson H.~L. {\&} Morgan W. W., 1953, ApJ, 117, 313
  
\bibitem[Joshi et al.(2012)Joshi et al.]{2012MNRAS...419..2379J}
  Joshi Y.~C., Joshi S., Kumar B., Mondal S. {\&} Balona L.~A.,  2012, MNRAS, 419, 2379

\bibitem[Joshi et al.(2014)Joshi et al.]{2014MNRAS...437..804J}
  Joshi Y.~C., Balona L.~A., Joshi S. {\&} Kumar B., 2014, MNRAS, 437, 804
  
\bibitem[Kaluzny \& Udalski(1992) Kaluzny \& Udalski]{1992AcA...42..49}
Kaluzny J. \& Udalski A., 1992, Acta Astron., 42, 49

\bibitem[Kharchenko et al.(2004)Kharchenko et al.]{2004AN...325..740K}
  Kharchenko N.~V., Piskunov A.~E., Roeser S., Schilbach E. {\&} Schola R.-D., 2004, Astron. Nachr., 325, 740
  
 \bibitem[Kharchenko et al.(2005)Kharchenko et al.]{2005A&A...438.1163K}
  Kharchenko N.~V., Piskunov A.~E., Roeser S., Schilbach E.  {\&} Schola R.-D., 2005, A{\&}A, 438, 1163

\bibitem[Lada \& Lada(2003)Lada \& Lada]{2003ARAA...41..57L}
  Lada C.~J. \& Lada E.~A., 2003, ARA\&A, 41, 57

\bibitem[Landolt(1992)Landolt]{1992AJ...104..340L}
  Landolt A.~U., 1992, AJ, 104, 340

\bibitem[Loktin \& Beshenov(2003)Loktin \& Beshenov]{2003AR...47..6L}
Loktin A.~V. {\&} Beshenov G.~V., 2003, Astron. Rep., 47, 6

\bibitem[Marigo et al.(2008)Marigo et al.]{2008AA...482..883M}
Marigo P., Girdardi L., Bressan A., et al., 2008, A{\&}A, 482, 883

\bibitem[Meuress(1958)Meuress]{1958AP...44..203M}
  Meuress J., 1958, Z Astrophysics, 44, 203

\bibitem[Moeder(1974)Moeder]{1974AA...32..177M}
  Moeder A., 1974, A{\&}A, 32, 177

\bibitem[Neckel \& Chini(1981)Neckel \& Chini]{1981AA...45..451N}
  Neckel T. {\&} Chini R., 1981, A{\&}A, 45, 451

\bibitem[Nilakshi et al.(2002)Nilakshi et al.]{2002AA...383..153N}
  Nilakshi, Sagar R., Pandey A. K. {\&} Mohan V., 2002, A{\&}A, 383, 153

\bibitem[Phleps \& Janes(1994)Phleps \& Janes]{1994AJ...90..31P}
Phelps R. L. {\&} Janes K. A., 1994, AJ, 90, 31

\bibitem[Ro$\ddot \texttt{e}$ser et al.(2010)Ro$\ddot \texttt{e}$ser et al.]{2010AJ...139..2440R}
Ro$\ddot \texttt{e}$ser S., Demliatnes M. {\&} Schibaon E., 2010, AJ, 139, 2440

\bibitem[Sanner et al.(2000)Sanner et al.]{2000AA...357..471S}
  Sanner J., Altmann M., Brunzendorf J. {\&} Geffert M., 2000, A{\&}A, 357, 471.

\bibitem[Schmidt-Kalar (1982)Schmidt-Kalar]{1982ND...26..14S}
  Schmidt-Kalar Th; 1982, In: Landolt/Bornestein, Numerical Data and functional Relationship in Science and Technology, New Series, Group VI, vol 26, Scaifers K., \& Voigt H. H.(eds.) Springer-Verlog, Berlin, p.14
  
\bibitem[Sharma et al.(2006)Sharma et al.]{2006AJ...132..1669S}
  Sharma S., Pandey A.~K., Ogura K., Mito H., Tarusawa K. {\&} Sager R., 2006, AJ, 132, 1669  

\bibitem[Sharma et al.(2008)Sharma et al.]{2008AJ...135..1934S}
  Sharma S., Pandey A.~K., Ogura K., Aoki T., Pandey K., Sandhu T.~S. {\&} Sager R., 2008, AJ, 135, 1934

 \bibitem[Skrutskie et al.(2006)Skrutskie et al.]{Skrutskie+2006}
 Skrutskie, M.~F., Cutri, R.~M., Stiening, R., et al., 2006, AJ, 131, 1163

\bibitem[Snedden et al.(1978)Snedden et al.]{1978APJ...223..168S}
  Snedden C., Gehrz R.~D., Hackwell J.~A., York D.~G. {\&} Snow T.~P., 1978, ApJ, 223, 168

\bibitem[Stetson(1987)Stetson]{1987PASP...99..191S}
  Stetson P. B., 1987, PASP, 99, 191

\bibitem[Stetson(1992)Stetson]{1992ASP...25..297S}
  Stetson P. B., 1992 in ASP conf. Ser. vol. 25, Astronomical Data Analysis Software and System, I. Astron. Soc. Pac., ed. Warrall D.~M., and Biemesderfer C., Barnes J., San Francisco, 297

\bibitem[Whittel {\&} van Breda(1980)Whittel {\&} van Breda]{1980MNRAS...192..467W}
 Whittel D.~C.~B. {\&} van Breda I.~G., 1980, MNRAS, 192, 467

\bibitem[Wright et al.(2010)Wright et al.]{2010AJ...140..1868W}
Wright E.~L., Eisenhardt P.~R.~M., Mainzer A.~K., et al., 2010, AJ, 140, 1868

\bibitem[Wu et. al.(2009)Wu et. al.]{2009MNRAS...399..214W}
Wu Z.~Y., Zhou X., Ma J. {\&} Du C.~H., 2009, MNRAS, 399, 2146

\bibitem[Zacharies et al.(2013)Zacharies et al.]{2013AJ...145..44Z}
Zacharies N., Finch C.~T., Girard T. M., Henden A., Bartlett J.~L., Monet D.~G. {\&} Zacharias M.~I., 2013, AJ, 145, 44

\end{thebibliography}

